MoBayes: A Modular Bayesian Framework for Separating Reasoning from Language in Conversational Clinical Decision Support

Large language models (LLMs) are increasingly used for conversational clinical decision support, yet they conflate next token prediction with probabilistic decision making. We argue that this conflation reflects an architectural limitation: such systems lack explicit posterior tracking, controllable abstention thresholds, and auditable reasoning chains. We introduce MoBayes, a Modular Bayesian dialogue framework that separates reasoning from language. The LLM acts only as a language interface, parsing patient conversation into structured observations, while a Bayesian module performs probabilistic inference over these observations to update posteriors, select follow-up questions via expected-information-gain and determine when to stop or defer through calibrated decision thresholds. This design enables explicit posterior tracking, controllable selective decision-making, and replaceable population-specific statistical backends without retraining the language model. Across empirical and LLM-generated knowledge bases, MoBayes outperforms standalone frontier LLM doctors, including matched model-family comparisons where inexpensive sensor models paired with MoBayes exceed larger autonomous models at lower cost. The advantage persists under adversarial patient communication styles and across varying diagnostic scenarios. These results suggest that reliable conversational clinical decision support systems should separate probabilistic reasoning from language generation rather than scaling model size alone. Code is available at https://anonymous.4open.science/r/MoBayes/

==> tables/tab_baseline_adaptations.tex <==
\addblock{
\begin{table}[t]
\centering

\caption{\replace{Baseline comparison across two benchmarks. \textbf{DDxPlus 50}: 50-patient curated subset with a 49-disease closed world, our PatientSim. \textbf{AgentClinic-MedQA}~\cite{schmidgall2024agentclinic}: 213-case USMLE-derived free-text dialogue benchmark with the AgentClinic patient and moderator agents. All non-fine-tuned methods use gpt-5.4-nano as the LLM backbone. \emph{Sel.\,Acc} = top-1 accuracy among committed predictions; \emph{Cov.} = fraction of patients on which the system commits (no abstention); \emph{DHS} is the harmonic mean of Sel.\,Acc and Cov ($\alpha{=}0.5$). Each method uses its own native abstention mechanism; for \ours we apply the DHS-optimal $\tau^*$ as in Table~\ref{tab:main}. All numbers are percentages. \\
$^{\dagger}$\,MEDDxAgent paper-best: PubMed retrieval + similarity-based (dynamic) 5-shot fewshot from a 500-patient validate-split pool, 3 iterations $\times$ 5 history-taking questions. \\
$^{\ddagger}$\,MEDDxAgent closed-world ablation (ours): local DDxPlus KB retrieval + random (static) 5-shot fewshot, otherwise identical.}{Baseline comparison on DDxPlus 50 (PatientSim) and AgentClinic-MedQA~\cite{schmidgall2024agentclinic}; non-fine-tuned methods use gpt-5.4-nano. Metrics in Eq.~\ref{eq:metrics}; \ours uses DHS-optimal $\tau^*$ as in Table~\ref{tab:main}. $^{\dagger}$\,MEDDxAgent paper-best (PubMed RAG + dynamic 5-shot, 3${\times}$5 turns); $^{\ddagger}$\,closed-world ablation (local KB + static 5-shot). Configurations in Appendix~\ref{app:baselines_protocol}.}}
\label{tab:baseline_adaptations}
\small
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.15}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}l ccccc @{\hskip 1.5em} ccccc@{}}
\toprule
& \multicolumn{5}{c}{\textbf{DDxPlus 50}} & \multicolumn{5}{c}{\textbf{AgentClinic-MedQA}} \\
\cmidrule(lr){2-6} \cmidrule(lr){7-11}
\textbf{Method} & Top-1 & Top-3 & Sel.\,Acc & Cov. & DHS & Top-1 & Top-3 & Sel.\,Acc & Cov. & DHS \\
\midrule
\multicolumn{11}{l}{\textit{Prompt-based}} \\
\midrule
Closed-World (CW)              & 42 & 68 & 62 & 68 & 65 & -- & -- & -- & -- & -- \\
Chain-of-Thought (CoT)         & 64 & 80 & 64 & 100 & 78 & -- & -- & -- & -- & -- \\
DDx-CoT                        & 46 & 80 & 70 & 66 & 68 & -- & -- & -- & -- & -- \\
Bayesian-CoT                   & 68 & 80 & 72 & 94 & 82 & -- & -- & -- & -- & -- \\
\midrule
\multicolumn{11}{l}{\textit{Information-pursuit}} \\
\midrule
UoT                            & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
\midrule
\multicolumn{11}{l}{\textit{Agent-based}} \\
\midrule
MediQ-Expert                   & 46 & -- & 46 & 100 & 63 & -- & -- & -- & -- & -- \\
MEDDxAgent\,---\,paper-best$^{\dagger}$        & 42 & 72 & 42 & 100 & 59 & -- & -- & -- & -- & -- \\
MEDDxAgent\,---\,closed-world ablation$^{\ddagger}$ & 44 & 74 & 44 & 100 & 61 & -- & -- & -- & -- & -- \\
\midrule
\multicolumn{11}{l}{\textit{Fine-tuned (specialised model)}} \\
\midrule
CoD / DiagnosisGPT-34B         & 14 & 22 & 14 & 100 & 25 & -- & -- & -- & -- & -- \\
\midrule
\multicolumn{11}{l}{\textit{Ours}} \\
\midrule
\textbf{\ours} (gpt-5.4-nano)   & \textbf{78} & \textbf{90} & \textbf{81} & \textbf{96}  & \textbf{88} & -- & -- & -- & -- & -- \\
\bottomrule
\end{tabular}%
}
\end{table}
}
